DiffVein: A Unified Diffusion Network for Finger Vein Segmentation and Authentication

Finger vein authentication, recognized for its high security and specificity, has become a focal point in biometric research. Traditional methods predominantly concentrate on vein feature extraction for discriminative modeling, with a limited exploration of generative approaches. Suffering from verification failure, existing methods often fail to obtain authentic vein patterns by segmentation. To fill this gap, we introduce DiffVein, a unified diffusion model-based framework which simultaneously addresses vein segmentation and authentication tasks. DiffVein is composed of two dedicated branches: one for segmentation and the other for denoising. For better feature interaction between these two branches, we introduce two specialized modules to improve their collective performance. The first, a mask condition module, incorporates the semantic information of vein patterns from the segmentation branch into the denoising process. Additionally, we also propose a Semantic Difference Transformer (SD-Former), which employs Fourier-space self-attention and cross-attention modules to extract category embedding before feeding it to the segmentation task. In this way, our framework allows for a dynamic interplay between diffusion and segmentation embeddings, thus vein segmentation and authentication tasks can inform and enhance each other in the joint training. To further optimize our model, we introduce a Fourier-space Structural Similarity (FourierSIM) loss function, which is tailored to improve the denoising network's learning efficacy. Extensive experiments on the USM and THU-MVFV3V datasets substantiates DiffVein's superior performance, setting new benchmarks in both vein segmentation and authentication tasks.

==> chap3/backup.tex <==
\section{Methods}

\subsection{Overview} \label{sec:overview}
\begin{figure*}[!htbp]
\centering
\includegraphics[width=\linewidth]{figs/chap3/overview.pdf}
\caption{The schematic illustration of DiffVein. \textcolor{red}{ADD LOSS AND LEGEND}}
\label{chap3:fig:overview}
\end{figure*}

\textcolor{blue}{
Fig.\ref{chap3:fig:overview} shows the overall architecture of our proposed network. As is shown in this figure, DiffVein contains two U-Net-like networks for denoising and segmentation branch. Given an image of the human finger captured by NIR camera, the segmentation branch mainly aims to localize the finger vein areas below the skin in the pixel-level and segment them in a binary mask. Besides, this network also serves as the feature extractor to generate the predicted feature embeddings for finger vein authentication task. The details of this network are presented in Sec.\ref{chap3:sec:segment}. After applying diffusion model on the embedding vectors mentioned above, the denoising branch is responsible for predicting the Gaussian noise added on the input noisy vectors and recovering the target information. Our diffusion model and denoising network is elaborated in Sec. \ref{chap3:sec:diffusion}. It should be noted that different schemes are used in the forward and reverse diffusion process. The upper and lower part of the framework illustrates the forward process for training and the reverse process for inference respectively. In this figure, the feature embeddings with more noise appear in darker colors than their counterparts with less noise. 
}

\textcolor{blue}{
The segmentation feature maps from the expanding path in Segmentation U-Net should be able to learn some high-level semantics information such as human tissue reflectivity, finger vein textures etc. The intuition of our work is that these clues are supposed to provide an important guidance to the denoising U-Net. Thus, we develop a mask condition module to introduce vein semantics to the denoising process, which is elaborated in Sec. \ref{chap3:sec:diffusion}. On the other hand, the denoising branch encodes the category information in an implicit manner. Our hypothesis is the segmentation task may potentially benefit from this additional category embedding because it helps the network to learn more distinctive features between different classes. Thus, the Semantic Difference Transformer (SD-Former) is proposed to extract semantic information from the denoising branch, and the details of this module are elaborated in Sec.\ref{chap3:sec:sdformer}. To sum up, mutual information will be flowed across both branches in a complementary way which boosts the overall performance.
}

\subsection{Segmentation Branch} \label{chap3:sec:segment}
\textcolor{blue}{
Given an input finger image $x$, the segmentation U-Net $\epsilon_s$ is responsible for predicting the binary vein mask $x_m$. $\epsilon_s$ is implemented by a UNet with modified input channels to reduce the computational burden. The contracting path in $S$ serves as a feature extractor and the detailed network structure is shown in Table \ref{chap3:tbl:seg_unet}. Note that \textbf{Convolution} in this table denotes the combination of convolution, batch normalization and ReLU activation, \textbf{Convolution*} denotes a composite layer with two \textbf{Convolution} stacked together. The output from block \textbf{Contract3} is represented as $s_1$, as illustrated in Fig. \ref{chap3:fig:overview}.
}
\begin{table}[htbp]
\caption{Network Configurations of Segmentation U-Net}
\renewcommand\arraystretch{1.5}
\begin{tabular}{c|ccc}
\hline
Block & Layer & Channel / Kernel / Stride & Output size \\ \hline
Conv0 & Convolution* & 16\ /\ 3\ /\ 1 & 16$\times$224$\times$224 \\ \hline
\multirow{2}{*}{Contract1} & Max Pooling & -\ /\ 2\ /\ 2 & \multirow{2}{*}{32$\times$112$\times$112} \\
 & Convolution* & 32\ /\ 3\ /\ 1 & \\ \hline
\multirow{2}{*}{Contract2} & Max Pooling & -\ /\ 2\ /\ 2 & \multirow{2}{*}{64$\times$56$\times$56} \\
 & \multicolumn{1}{l}{Convolution*} & 64\ /\ 3\ /\ 1 & \\ \hline
\multirow{2}{*}{Contract3} & Max Pooling & -\ /\ 2\ /\ 2 & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}128$\times$28$\times$28\\ ($s_1$)\end{tabular}} \\
 & \multicolumn{1}{l}{Convolution*} & 128\ /\ 3\ /\ 1 & \\ \hline
\multirow{2}{*}{Expand1} & Up Sampling & -\ /\ 2\ /\ - & \multirow{2}{*}{64$\times$56$\times$56} \\
 & \multicolumn{1}{l}{Convolution*} & 64\ /\ 3\ /\ 1 \\ \hline
\multirow{2}{*}{Expand2} & Up Sampling & -\ /\ 2\ /\ - & \multirow{2}{*}{32$\times$112$\times$112} \\
 & \multicolumn{1}{l}{Convolution*} & 32\ /\ 3\ /\ 1 & \\ \hline
\multirow{2}{*}{Expand3} & Up Sampling & -\ /\ 2\ /\ - & \multirow{2}{*}{16$\times$224$\times$224} \\
 & \multicolumn{1}{l}{Convolution*} & 16\ /\ 3\ /\ 1 & \\ \hline
Out & Convolution & 1\ /\ 1\ /\ 1 & 1$\times$224$\times$224 \\ \hline
\end{tabular}
\label{chap3:tbl:seg_unet}
\end{table}

For authentication task, feature embedding from bottleneck layer is projected into matching space by stacked fully-connected layers before predicting the final matching vectors. The goal of authentication task is to enlarge the distance of matching vectors between different classes, therefore circle loss as shown in Eq. \cite{sun2020circle} is used to supervision this task:
\begin{align}
\mathcal{L}_{auth} = log[1+
& \sum^{L}_{j=1}exp(\gamma\alpha^{j}_{n}(s^{j}_{n}-\Delta_{n})) \\ \notag
& \sum^{K}_{i=1}exp(-\gamma\alpha^{i}_{p}(s^{i}_{p}-\Delta_{p}))] 
\end{align}
where $L$ and $K$ is the number of matches; $s_p$ and $s_n$ denote the cosine similarity of matching vectors within the same class and across the different classes respectively; $\alpha_p$ and $\alpha_n$ is the hyper-parameters to regulate the weights of the gradients of $s_p$ and $s_n$; $\gamma$ is the hyper-parameter.

In expanding path, convolution layers with upsampling module are utilized to generate the final vein texture segmentation result. This segmentation task is supervised by cross entropy and Dice loss, formulated as Eq.\ref{eq:seg_loss}.
\begin{equation}
\mathcal{L}_{seg} = \mathcal{L}_{Dice} + \alpha \mathcal{L}_{CE}
\label{eq:seg_loss}
\end{equation}

\subsection{Diffusion Model and Denoising Branch} \label{chap3:sec:diffusion}
\textcolor{red}{TO POLISH} 
Following the standard implementation of DDPM\cite{ho2020denoising, yang2023diffmic}, the diffusion model in this paper includes both a forward process for training and an inverse process for evaluation and inference. In the training stage, the matching vectors $\hat{y}^{v}$ generated from the segmentation branch is added by Gaussian noise through the diffusion process conditioned by time step $t$ sampled from a uniform distribution of $\left [1, T \right ]$ to form the noisy vectors $\left \{ y_1^v, y_2^v, \cdots, y_T^v \right \}$ following:
\begin{equation}
y_t =\sqrt{\bar{\alpha}_t}y_0 + \sqrt{1-\bar{\alpha}_t}\epsilon + (1-\sqrt{\bar{\alpha}_t})(\hat{y_g}+\hat{y_l})
\label{eq:diffusion}
\end{equation}
where, $\epsilon \sim \mathcal{N}(0,I)$;$\bar{\alpha }_t=  {\textstyle \prod_{t}}\alpha_t $;$\alpha_t=1-\beta_t$ denotes the linear noise scheduling strategy;$\left \{ \beta_t \right \}_{t=1:T} \in (0,1)^T$. Then, these 1-D vectors are projected to 2-D feature maps in the latent space for the sake of further computation. The denoising network is implemented by a UNet to learn the noise distribution and parameterize the reverse diffusion process. The outputs from denosing network are inversely projected into 1-D matching vectors for computing loss.

In the inference stage, the final predicted matching vectors $\hat{y}^0$ are obtained by transforming the noisy distribution $p_{\theta}(y_T)$ to the predefined noise distribution $p_{\theta}(y_0)$ through the trained UNet $\epsilon_{\theta}$. This process can be formulated as Eq.\ref{eq:denosing:1}-\ref{eq:denoising:2} shown below:
\begin{equation}
    p_{\theta}(y_{0:T-1}|y_{T},\rho(x))=\prod _{t=1}^{T}p_{\theta}(y_{t-1}|y_{t},\rho(x))
    \label{eq:denoising:1}
\end{equation}
\begin{equation}
    p_{\theta}(y_T)=\mathcal{N}(\frac{1}{2}, I)
    \label{eq:denosing:2}
\end{equation}
where $\theta$ is the parameters of the denosing UNet, $\mathcal{N}(\cdot, \cdot)$ denotes the normal distribution, and $I$ is the identity matrix.

\subsection{Semantic Difference Transformer} \label{chap3:sec:sdformer}
\textcolor{red}{TO POLISH}

We propose a novel transformer architecture, called Spectrum-Space Transformer (SS-Former), to effectively integrate the conditional segmentation embedding into the diffusion embedding. SS-Former is composed of several blocks that share the same architecture. Each block consists of two cross-attention like modules. The first encodes the diffusion noise embedding into the condition semantic embedding, and the next module encodes the noise-blended semantic embedding into the diffusion noise embedding. This allows the model to learn the interaction between noise and semantic features and achieve a stronger representation.

Since the Diffusion Model predicts the redundant noise from the noisy mask input, it will have a domain gap between its embedding and that of the conditional segmentation semantic embedding. This gap can lead to confusion when using matrix manipulations in a stranded transformer. To address this challenge, we propose a novel spectrum-space attention mechanism. The key idea is to merge semantic and noise information in Fourier space, rather than Euclidean space. This allows for the separation and blending of components based on frequency-affinity in different spectrums. Formally, consider c0 is the deepest feature embedding of Condition Model and e is that of Diffusion Model. We first transfer c0 and e to the Fourier space, denoted as F(c0) and F(e), respectively.
\begin{equation}
    \mathcal{M}=asin(w(F(c^0)\mathcal{W}^q)
\end{equation}

\begin{figure}[!htbp]
\centering
\begin{minipage}{0.95\linewidth}\centering
\includegraphics[width=0.9\textwidth]{figs/chap3/self-attention.pdf}
\centerline{(a) Fourier space self-attention module}
\end{minipage}
\begin{minipage}{0.95\linewidth}\centering
\includegraphics[width=0.9\textwidth]{figs/chap3/cross-attention.pdf}
\centerline{(b) Fourier space cross-attention module}
\end{minipage}
\label{chap4:fig:attention}
\caption{Schematic illustration of our proposed method.}
\end{figure}

Note that the feature maps are all patchlized and liner projected in accordance with the standard vision transformer method. Then we compute an affinity weight map over Fourier space taking e as the query and c0 as the key, as represented by the following equation:
\begin{figure}[!htbp]
\centering
\includegraphics[width=0.8\linewidth]{figs/chap3/former.pdf}
\caption{Schematic illustration of our proposed method.}
\label{chap4:fig:former}
\end{figure}

\subsection{Training and Inference Scheme}
The diffusion model in this study leverages a standard DDPM training process, where the diffusion time step t is selected from a uniform distribution of $\left [ 1, T \right ]$, and the noise is linearly scheduled with $\beta_{1}=1\times10^{-4}$ and $\beta_{T}=0.02$. We adopt ResNet18 as the image encoder, Following [12], we concatenate, and apply a linear layer with an output dimension of 6144 to obtain the fused vector in the latent space. To condition the response embedding on the timestep, we perform a Hadamard product between the fused vector and a timestep embedding. We then integrate the image feature embedding and response embedding by performing another Hadamard product between them. The output vector is sent through two consecutive fully-connected layers, each followed by a Hadamard product with a timestep embedding. 

Finally, we use a fully-connected layer to predict the noise with an output dimension of classes. It is worth noting that all fully-connected layers are accompanied by a batch normalization layer and a Softplus non-linearity, with the exception of the output layer. For the DCG model D, the backbone of its global and local stream is ResNet. We adopt the standard cross-entropy loss as the objective of the DCG model. We jointly train the denoising diffusion model and DCG model after pretraining the DCG model 10 epochs for warm-up, thereby resulting in an end-to-end DiffMIC for medical image classification.

==> chap3/training_scheme.tex <==
\subsection{Training and Inference Scheme}
The diffusion model in this study leverages a standard DDPM training process, where the diffusion time step t is selected from a uniform distribution of $\left [ 1, T \right ]$, and the noise is linearly scheduled with $\beta_{1}=1\times10^{-4}$ and $\beta_{T}=0.02$. We adopt ResNet18 as the image encoder, Following [12], we concatenate, and apply a linear layer with an output dimension of 6144 to obtain the fused vector in the latent space. To condition the response embedding on the timestep, we perform a Hadamard product between the fused vector and a timestep embedding. We then integrate the image feature embedding and response embedding by performing another Hadamard product between them. The output vector is sent through two consecutive fully-connected layers, each followed by a Hadamard product with a timestep embedding. 

Finally, we use a fully-connected layer to predict the noise with an output dimension of classes. It is worth noting that all fully-connected layers are accompanied by a batch normalization layer and a Softplus non-linearity, with the exception of the output layer. For the DCG model D, the backbone of its global and local stream is ResNet. We adopt the standard cross-entropy loss as the objective of the DCG model. We jointly train the denoising diffusion model and DCG model after pretraining the DCG model 10 epochs for warm-up, thereby resulting in an end-to-end DiffMIC for medical image classification.

==> chap4/chap4_backup.tex <==
\section{Experiments}
\textcolor{blue}{DONE!!}

In this section, extensive experiments are conducted on USM and THU-MVFV3V dataset and both finger vein segmentation and authentication results are provided to validate our proposed method. We elaborate the details of datasets and the generation of vein masks in the Sec. \ref{chap4:sec:dataset}. We also summarize the key index of the datasets in Table \ref{chap4:tbl:datasets}. Our implementation details and evaluation metrics are provided in Sec. \ref{chap4:sec:settings}. Comparative experiments and analysis are presented in Sec. \ref{chap4:sec:auth} and \ref{chap4:sec:seg}. Also, we designed a series of ablation experiments to further study the effectiveness of our proposed modules, which can be seen in Section \ref{chap4:sec:ablation}.
\begin{table}[htbp]
\centering
\caption{Details of Finger Vein Datasets}
\renewcommand\arraystretch{1.5}
\begin{tabular}{c|cc}
\hline
Dataset & USM \cite{asaari2014fusion} & THU-MVFV3V \cite{zhao2023vpcformer} \\ \hline
Finger type & Middle \& Index & Middle \& Index \\ \hline
ROI size & 300$\times$100 & 300$\times$150 \\ \hline
Number of subjects & 492 & 660 \\ \hline
\makecell[c]{Number of samples\\per finger} & 6 & 6 \\ \hline
\makecell[c]{Number of total\\images in use} & 5904 & 7920 \\ \hline
\end{tabular}
\label{chap4:tbl:datasets}
\end{table}

%% ===================================================
%% ===================================================
%% THIS IS THE BEGINING OF A NEW SUB-SECTION
\subsection{Datasets \label{chap4:sec:dataset}}
\subsubsection{USM Dataset}
\textcolor{blue}{DONE!!}

USM \cite{asaari2014fusion} dataset was constructed by the research team from Universiti Sains Malaysia in 2014. This dataset includes a collection of finger vein images from 123 volunteers and each of them provided their index and middle fingers of both hands. Each finger was captured for 6 times in two separate sessions with a time interval of more than two weeks. Therefore, there are 492 finger categories with a total of 5904 finger vein images in this dataset. The resolution of raw images is 640$\times$480 pixels and a region of interest (ROI) with a size of 300$\times$100 is also provided for each raw finger vein image, as illustrated in Fig. \ref{chap4:fig:usm_dataset} (a).

In order to supervise the segmentation task, the mask generation module (MGM) in EIFNet \cite{song2022eifnet} was used here to generate the finger vein mask. We trained the MGM on the THU-FVS dataset with human-annotated vein masks and followed the default settings as advised in EIFNet to generate the vein masks of USM dataset. An example vein mask is presented in Fig. \ref{chap4:fig:usm_dataset} (c).
\begin{figure}[htbp]
\centering
\begin{minipage}{0.4\linewidth}\centering
\includegraphics[width=\linewidth]{figs/chap4/dataset/usm_roi.png}
\centerline{(a)}
\end{minipage}
\hspace{5pt}
\begin{minipage}{0.4\linewidth}\centering
\includegraphics[width=\linewidth]{figs/chap4/dataset/usm_mask.png}
\centerline{(b)}
\end{minipage}
\caption{A sample of USM dataset. (a) ROI image; (b) Vein mask.}
\label{chap4:fig:usm_dataset}
\end{figure}

\subsubsection{THU-MVFV3V Dataset}
\textcolor{blue}{DONE!!}

THU-MVFV3V \cite{zhao2023vpcformer} dataset was established by Tsinghua University in 2023. The images in this dataset were collected from 92 males and 79 females. Each volunteer provided their index and middle fingers from both hands and the total number of finger categories is 660 after leaving out poorly-captured samples. Similarly, the data acquisition process included two phases with a time span of 45.8 days in average. Each finger was sampled 6 times at three angles (-45$^{\circ}$, 0$^{\circ}$, 45$^{\circ}$) in each session, resulting in a total of 23,760 finger vein images. It should be noted that only the images from center angle (0$^{\circ}$) are used in our work, which means 7920 images are used in the following experiments. A 300$\times$150 ROI is also provided for each image.

Since no human correlation was involved in the learning-based vein mask generation, we combined the segmentation results of EIFNet with those of other three explicit vein extraction methods LMC \cite{miura2007extraction}, EMC \cite{syarif2017enhanced}, Gabor filter \cite{kumar2011human} and adopted the majority vote algorithm (MVA) to generate the vein masks for THU-MVFV3V dataset. Firstly, each of the algorithms generate their predicted mask separately. When a pixel is labeled as a vein point in more than three predicted masks, then this pixel can be regarded as a reliable vein point. Otherwise, this pixel should be labelled as background. Fig. \ref{chap4:fig:THUMVFV3V_dataset} shows the vein masks predicted by different methods and our final results by MVA.
\begin{figure}[htbp]
\centering
\begin{minipage}{0.15\linewidth}\centering
\includegraphics[width=\linewidth]{figs/chap4/dataset/THUMVFV3V_roi.png}
\centerline{(a)}
\end{minipage}
\begin{minipage}{0.15\linewidth}\centering
\includegraphics[width=\linewidth]{figs/chap4/dataset/THUMVFV3V_lmc.png}
\centerline{(b)}
\end{minipage}
\begin{minipage}{0.15\linewidth}\centering
\includegraphics[width=\linewidth]{figs/chap4/dataset/THUMVFV3V_emc.png}
\centerline{(c)}
\end{minipage}
\begin{minipage}{0.15\linewidth}\centering
\includegraphics[width=\linewidth]{figs/chap4/dataset/THUMVFV3V_gabor.png}
\centerline{(d)}
\end{minipage}
\begin{minipage}{0.15\linewidth}\centering
\includegraphics[width=\linewidth]{figs/chap4/dataset/THUMVFV3V_eifnet.png}
\centerline{(e)}
\end{minipage}
\begin{minipage}{0.15\linewidth}\centering
\includegraphics[width=\linewidth]{figs/chap4/dataset/THUMVFV3V_mask.png}
\centerline{(f)}
\end{minipage}
\caption{A sample of THU-MVFV3V dataset. (a) ROI image; (b) Vein mask by LMC; (c) Vein mask by EMC; (d) Vein mask by Gabor filter; (e) Vein mask by EIFNet; (f) Final vein mask.}
\label{chap4:fig:THUMVFV3V_dataset}
\end{figure}

%% ===================================================
%% ===================================================
%% THIS IS THE BEGINING OF A NEW SUB-SECTION
\subsection{Experimental Settings \label{chap4:sec:settings}}
\subsubsection{Implementation Details}
\textcolor{blue}{DONE!!}

Our framework is implemented with PyTorch on a single NVIDIA RTX 3090 GPU. Before the training process, we randomly cropped a square area on each ROI image and its corresponding binary mask. Then we resize their resolution to $224\times224$ to adapt to our network. Random change in contrast and Gaussian blur are applied on the training images for data augmentation.

In the training phase, the initial learning rate for the segmentation and denoising U-Net are set as $1\times10^{-4}$ and $1\times10^{-3}$ respectively. The entire framework was trained in an end-to-end manner using the AdamW optimizer. It should be noted that following the training scheme in \cite{yang2023diffmic}, the segmentation branch needs to be pre-trained at first to provide a preliminary prediction before training the entire framework jointly. The pre-training epoch is set as 20 epochs and the number of total training epochs is set as 1000 for both datasets. The batch size is set as 4 for both pre-training and joint-training. Following the common practice in this field \cite{song2022eifnet,zhao2023vpcformer}, we split the dataset into the training and testing set according to the data acquisition session and data from session one is used for training while data from session two is used for evaluation.

In the inference phase, based on the empirical data in \cite{yang2023diffmic} and our experimental results, we set the total diffusion time step $T$ as 100 for USM dataset and 200 for THU-MVFV3V dataset.

\subsubsection{Evaluation Metrics}
\textcolor{blue}{DONE!!}

To evaluate the segmentation and authentication performance of our proposed method, we adopted several mainstream metrics for fair comparison with other popular methods. Both verification and identification tasks are included in finger vein authentication.

EER, as a widely used metrics in biometric recognition, is used here to evaluate the matching performance between the training and testing test, which we term as finger vein verification task in this paper. In the detection error tradeoff (DET) \cite{martin1997det} curve, EER represents the intersection where false acceptance rate (FAR) coincides with false rejection rate (FRR). We provide both DET curve and EER value in the following experiments for comprehensive analysis. 

ACC is a commonly-used metrics for classification tasks and it is used here to evaluate the prediction performance, which we term as finger vein identification task. Different from EER, ACC only evaluate the accuracy of predicted finger categories in the testing test. 

For finger vein segmentation, we adopted a series of volumetric scores including mean Dice coefficient (Dice), centerline Dice (clDice) \cite{shit2021cldice}, accuracy (ACC) and AUC to evaluate the overall segmentation performance. It should be noted that clDice is more suitable here since it evaluates the result from the perspective of topological continuity and the veins inside a finger are inherently tubular structures.

%% ===================================================
%% ===================================================
%% THIS IS THE BEGINING OF A NEW SECTION
\subsection{Finger Vein Authentication \label{chap4:sec:auth}}
\textcolor{blue}{DONE!!}

In this section, we compared the authentication performance of DiffVein with those of several widely-used traditional and deep learning-based methods on USM and THU-MVFV3V datasets. Both verification and identification tasks are included in our experiments. 

\textcolor{blue}{
The DET curves of comparative experiments on both datasets are shown in Fig. \ref{chap4:fig:usm_auth} and Fig. \ref{chap4:fig:thumvfv3v_auth}. It can be seen from Fig. \ref{chap4:fig:usm_auth} that CAE, EIFNet and our DiffVein significantly outperform other methods, where our method slightly leads the other two opponents. THU-MVFV3V dataset is more complicated than USM so the distinction of performance between different methods is more remarkable. As can be observed in Fig. \ref{chap4:fig:thumvfv3v_auth}, the DET curve of our method is consistently lower than that of VPCFormer and HCAN proposed in recent years, which indicates our method outperform the other existing methods.
}
%% USM Dataset
\begin{figure}[!htbp]
\centering
\includegraphics[width=0.85\linewidth]{figs/chap4/auth/det_usm.png}
\caption{DET curve of different method on USM dataset.}
\label{chap4:fig:usm_auth}
\end{figure}
%% THU-MVFV3V Dataset
\begin{figure}[!htbp]
\centering
\includegraphics[width=0.85\linewidth]{figs/chap4/auth/det_thumvfv.png}
\caption{DET curve of different method on THU-MVFV3V dataset.}
\label{chap4:fig:thumvfv3v_auth}
\end{figure}

\textcolor{blue}{
More quantitative results are shown in Table \ref{chap4:tbl:usm_auth} and Table \ref{chap4:tbl:thumvfv3v_auth}. The best results are highlighted in bold. It can be observed that learning-based methods generally performs better than traditional methos under the EER and ACC metrics on both of the datasets. It means that these methods are prone to predict more consistent intra-class features and more accurate inter-class features, which validates the powerful capacity of CNN-based deep networks in extracting inherent and implicit patterns. Our DiffVein shows the leading performance across all the other methods, since it fully exploits the advantage of mask condition and diffusion model. Predicting the Gaussian noise by conditioning with segmentation feature maps can make the denoising network converge more easily, which leads to considerable performance boost. The further ablation analysis on the effectiveness of diffusion model and mask condition is elaborated in Sec. \ref{chap4:sec:ablation}.
}
% USM DATASET
\begin{table}[htbp]
\centering
\caption{Comparison of Authentication Results of Different Methods on USM dataset}
\renewcommand\arraystretch{1.5}
\setlength{\tabcolsep}{0.03\columnwidth}
\begin{tabular}{c|l|cc}
\hline
Type & Method & EER(\%) & ACC(\%)\\ \hline
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Traditional\\ methods\end{tabular}}  
& RLT \cite{miura2004feature} & 6.73 &  92.04 \\ 
& LMC \cite{miura2007extraction} & 4.04 &  97.01 \\
& PC \cite{choi2009finger} & 4.34 &  96.87 \\
& WLD \cite{huang2010finger} & 4.41 &  96.55 \\
& Gabor filters \cite{kumar2011human} & 3.47 &  97.32 \\
& EMC \cite{syarif2017enhanced} & 1.63 &  98.42 \\
& ASAVE \cite{yang2017finger} & 5.14 &  95.01 \\
& LBP \cite{lee2009finger} & 5.76 &  95.48 \\ \hline
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}Learning-based\\ methods\end{tabular}} 
& CNN+FCN \cite{qin2017deep} & 1.42 &  98.41 \\
& CAE \cite{hou2019convolutional} & 0.12 &  99.54 \\
& FVRAS-Net \cite{yang2020fvras} & 0.95 &  98.81 \\
& Lightweight CNN \cite{zhao2020finger} & 1.07 &  98.53 \\
& Dynamic softmax \cite{li2022improving} & 0.81 &  98.79 \\
& EIFNet \cite{song2022eifnet} & 0.10 &  99.76   \\ \cline{2-4} 
& \textbf{Ours}   & \textbf{0.08} & {\textbf{99.79}}  \\ \hline
\end{tabular}
\label{chap4:tbl:usm_auth}
\end{table}

%% THUMVFV
\begin{table}[htbp]
\centering
\caption{Comparison of Authentication Results of Different Methods on THU-MVFV3V dataset}
\renewcommand\arraystretch{1.5}
\setlength{\tabcolsep}{0.04\columnwidth}
\begin{tabular}{c|l|cc}
\hline
Type & Method & EER(\%) & ACC(\%) \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Traditional\\ methods\end{tabular}} 
& LMC \cite{miura2007extraction} & 7.65  &  91.13 \\
& WLD \cite{huang2010finger} & 5.64  &  95.51 \\
& LDC \cite{meng2012finger} & 6.05  &  92.73 \\
& Gabor filters \cite{kumar2011human} & 8.68  &  90.88 \\
& PWBDC \cite{yang2019hybrid} & 7.56 &  91.03 \\ \hline
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Learning-based\\ methods\end{tabular}} 
& ResNet50 \cite{resnet} & 1.23  & 98.23 \\
& ECANet \cite{wang2020eca} & 0.98  & 98.82 \\
& MRFBCNN \cite{wang2021finger} & 0.92  & 98.76 \\
& ArcVein \cite{hou2021arcvein} & 2.45  & 96.97 \\
& ViT \cite{dosovitskiy2020vit} & 1.56  & 98.89 \\
& HCAN \cite{zhao2022exploiting} & 0.68  & 99.44 \\
& VPCFormer \cite{zhao2023vpcformer} & 0.45  & \textbf{99.67} \\ \cline{2-4} 
& \textbf{Ours} & \textbf{0.33} & 99.65    \\ \hline
\end{tabular}
\label{chap4:tbl:thumvfv3v_auth}
\end{table}

%% ===================================================
%% ===================================================
%% THIS IS THE BEGINING OF A NEW SECTION
\subsection{Finger Vein Segmentation \label{chap4:sec:seg}}
We compare our proposed method with other general segmentation methods including U-Net \cite{cciccek20163d}, TransUNet \cite{chen2021transunet} and methods designed especially for tubular structure segmentation including DCU-Net \cite{yang2022dcu}, DSCNet \cite{qi2023dynamic}. The volumetric scores are listed in Table \ref{chap4:tbl:all_seg} and the best results are highlighted in bold. It can be seen in the table that DSCNet and our segmentation network clearly outperform other methods in all of the volumetric scores on both datasets.

It should be noted that finger vein segmentation is some kind of auxiliary task in our entire framework, so technically our goal is not to generate vein masks which are as similar to groundtruth masks as possible, especially given that the groundtruth veins used in our paper does not represent the location and geometry of all finger veins correctly. Instead, we seek to generate more meaningful and representative vein masks which is capable of boosting the finger authentication process.

\begin{table*}[htbp]
\centering
\caption{Comparison of Segmentation Results of Different Methods on THU-MVFV3V Dataset}
\renewcommand\arraystretch{1.5}
\setlength{\tabcolsep}{0.055\columnwidth}
\begin{tabular}{c|c|ccccc}
\hline
Dataset & Method & Dice(\%) & clDice(\%) & ACC(\%) & AUC(\%) & mIoU(\%) \\ \hline
\multirow{4}{*}{USM} 
& UNet \cite{cciccek20163d} & 79.17 & 79.17 & 79.17 & 79.17 & 79.17 \\
& TransUNet \cite{chen2021transunet} & 82.01 & 82.01 & 82.01 & 82.01 & 82.01 \\
& DCU-Net \cite{yang2022dcu} & 84.02 & 84.02 & 84.02 & 84.02 & 84.02 \\ \cline{2-7}
& \textbf{Ours} & \textbf{86.26} & \textbf{86.26} & \textbf{86.26} & \textbf{86.26} & \textbf{86.26} \\ \hline
\multirow{4}{*}{THU-MVFV3V} 
& UNet \cite{cciccek20163d} & 79.17 & 79.17 & 79.17 & 79.17 & 79.17 \\
& TransUNet \cite{chen2021transunet} & 82.01 & 82.01 & 82.01 & 82.01 & 82.01 \\
& DCU-Net \cite{yang2022dcu} & 84.02 & 84.02 & 84.02 & 84.02 & 84.02 \\ \cline{2-7}
& \textbf{Ours} & \textbf{86.26} & \textbf{86.26} & \textbf{86.26} & \textbf{86.26} & \textbf{86.26} \\ \hline
\end{tabular}
\label{chap4:tbl:all_seg}
\end{table*}

The visual results of different methods on THU-MVFV3V dataset and USM dataset are shown in Fig. \ref{chap4:fig:thumvfv3v_seg} and Fig. \ref{chap4:fig:usm_seg} respectively.
It can be seen that vein masks in THU-MVFV are generally thin and disperse because only the vein pixels with high reliability selected by MVA are finally considered as valid vein masks. On the other hand, USM masks are generally thick and continuous. This characteristic is mainly attributed to the human-annotated masks used in the training of EIFNet. Clear, these two datasets pose different kinds of dataset, which is quite challenging when evaluating the overall performance of the segmentation methods. 

It can be seen from Fig. \ref{chap4:fig:thumvfv3v_seg} that, all of the listed methods are good at segmenting those long, continuous and thick veins while performing distinctly when it comes to thin and short veins. In Row No.1, our method excels at understanding the structure of the isolated vein sections highlighted by red box. In Row No.2, our method obtain the best performance connecting the thin, fragile section in the bed rox.

As illustrated in Fig. \ref{chap4:fig:usm_seg}, all of the predicted vein masks well captures the general topological structure of finger veins but addresses the interconnection of vein streams differently. In Row No.1, the groundtruth mask indicates that the veins in the red box should form an annular shape and only our method presents this characteristic correctly. In Row No.2, the vein starting from the left corner of the red box should bifurcate into two continuous streams. The other methods fail to understand this bifurcation while the predicted mask by our method has the best visual effect.

To sum up, although the masks generated by these methods take into account the geometric structure information such as the width and direction of the vein stripe, our DiffVein generates veins with better continuity and by leaving out those inessential and isolated vein patch.

\begin{figure*}[htbp]
\centering
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[height=0.055\textheight]{figs/chap4/thumvfv3v_seg/raw100.png}
\centerline{\quad}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[height=0.055\textheight]{figs/chap4/thumvfv3v_seg/gt100.png}
\centerline{\quad}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[height=0.055\textheight]{figs/chap4/thumvfv3v_seg/unet100.png}
\centerline{\quad}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[height=0.055\textheight]{figs/chap4/thumvfv3v_seg/transunet100.png}
\centerline{\quad}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[height=0.055\textheight]{figs/chap4/thumvfv3v_seg/dcunet100.png}
\centerline{\quad}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[height=0.055\textheight]{figs/chap4/thumvfv3v_seg/ours100.png}
\centerline{\quad}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[height=0.055\textheight]{figs/chap4/thumvfv3v_seg/raw545.png}
\centerline{(a)}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[height=0.055\textheight]{figs/chap4/thumvfv3v_seg/gt545.png}
\centerline{(b)}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[height=0.055\textheight]{figs/chap4/thumvfv3v_seg/unet545.png}
\centerline{(c)}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[height=0.055\textheight]{figs/chap4/thumvfv3v_seg/transunet545.png}
\centerline{(d)}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[height=0.055\textheight]{figs/chap4/thumvfv3v_seg/dcunet545.png}
\centerline{(e)}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[height=0.055\textheight]{figs/chap4/thumvfv3v_seg/ours545.png}
\centerline{(f)}
\end{minipage}
\caption{Visualization of finger vein segmentation results on THU-MVFV3V dataset using different methods: (a) ROI image; (b) Groundtruth mask; (c) UNet; (d) TransUNet; (e) DCUNet; (f) Ours.}
\label{chap4:fig:THU-MVFV3V_seg}
\end{figure*}

\begin{figure*}[htbp]
\centering
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[width=0.95\linewidth]{figs/chap4/usm_seg/raw101.png}
\centerline{\quad}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[width=0.95\linewidth]{figs/chap4/usm_seg/gt101.png}
\centerline{\quad}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[width=0.95\linewidth]{figs/chap4/usm_seg/unet101.png}
\centerline{\quad}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[width=0.95\linewidth]{figs/chap4/usm_seg/transunet101.png}
\centerline{\quad}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[width=0.95\linewidth]{figs/chap4/usm_seg/dcunet101.png}
\centerline{\quad}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[width=0.95\linewidth]{figs/chap4/usm_seg/ours101.png}
\centerline{\quad}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[width=0.95\linewidth]{figs/chap4/usm_seg/raw101.png}
\centerline{(a)}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[width=0.95\linewidth]{figs/chap4/usm_seg/gt101.png}
\centerline{(b)}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[width=0.95\linewidth]{figs/chap4/usm_seg/unet101.png}
\centerline{(c)}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[width=0.95\linewidth]{figs/chap4/usm_seg/transunet101.png}
\centerline{(d)}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[width=0.95\linewidth]{figs/chap4/usm_seg/dcunet101.png}
\centerline{(e)}
\end{minipage}
\begin{minipage}{0.16\linewidth}\centering
\includegraphics[width=0.95\linewidth]{figs/chap4/usm_seg/ours101.png}
\centerline{(f)}
\end{minipage}
\caption{Visualization of finger vein segmentation results on USM dataset using different methods: (a) ROI image; (b) Groundtruth mask; (c) UNet; (d) TransUNet; (e) DCUNet; (f) Ours.}
\label{chap4:fig:usm_seg}
\end{figure*}

%% ===================================================
%% ===================================================
%% THIS IS THE BEGINING OF A NEW SECTION
\subsection{Ablation Study \label{chap4:sec:ablation}}

\begin{table*}[htbp]
\centering
\caption{Ablation study}
\renewcommand\arraystretch{1.5}
\setlength{\tabcolsep}{0.055\columnwidth}
\begin{tabular}{c|ccc|ccc}
\hline
Combinations & Diffusion    & FD Loss      & SD-Former    & Dice(\%) & EER(\%) & ACC(\%) \\ \hline
Basic        & -            & -            & -            & 82.37    & 82.37   & 82.37   \\
$C_1$        & $\checkmark$ & -            & -            & 82.37    & 82.37   & 82.37   \\
$C_2$        & $\checkmark$ & $\checkmark$ & -            & 82.37    & 82.37   & 82.37   \\
$C_3$        & $\checkmark$ & -            & $\checkmark$ & 82.37    & 82.37   & 82.37   \\
Full         & $\checkmark$ & $\checkmark$ & $\checkmark$ & 82.37    & 82.37   & 82.37   \\ \hline
\end{tabular}
\label{chap4:fig:ablation}
\end{table*}

Extensive experiments are conducted to evaluate the effectiveness of major modules of our network. To do so, we build three baseline networks from our method. The first baseline (denoted as “basic”) is to remove
all diffusion operations and the MMD regularization loss from our network. It means that “basic” is equal to the classical ResNet18. Then, we apply the vanilla diffusion process onto “basic” to construct another baseline network (denoted as “C1”), and further add our dual-granularity conditional guidance into the diffusion process to build a baseline network, which is denoted as “C2”. Hence, “C2” is equal to removing the MMD regularization loss from our network for image classification. Table 2 reports the Accuracy and F1-score results of our method and three baseline networks on our PMG2000 dataset. Apparently, compared to “basic”, “C1” has an Accuracy improvement of 0.027 and an F1-score improvement of 0.018, which indicates that the diffusion mechanism can learn more discriminate features for medical image classification, thereby improving the PMG performance. Moreover, the better Accuracy and F1-score results of “C2” over “C1” demonstrates that introducing our dual-granularity conditional guidance into the vanilla diffusion process can benefit the PMG performance. Furthermore, our method outperforms “C2” in terms of Accuracy and F1-score, which indicates that exploring the MMD regularization loss in the diffusion process can further help to enhance the PMG results.
